Chem3DLLM: 3D Multimodal Large Language Models for Chemistry

In the real world, a molecule is a 3D geometric structure. Compared to 1D SMILES sequences and 2D molecular graphs, 3D molecules represent the most informative molecular modality. Despite the rapid progress of autoregressive-based language models, they cannot handle the generation of 3D molecular conformation due to several challenges: 1) 3D molecular structures are incompatible with LLMs' discrete token space, 2) integrating heterogeneous inputs like proteins, ligands, and text remains difficult within a unified model, and 3) LLMs lack essential scientific priors, hindering the enforcement of physical and chemical constraints during generation. To tackle these issues, we present Chem3DLLM, a unified protein-conditioned multimodal large language model. Our approach designs a novel reversible text encoding for 3D molecular structures using run-length compression, achieving 3x size reduction while preserving complete structural information. This enables seamless integration of molecular geometry with protein pocket features in a single LLM architecture. We employ reinforcement learning with stability-based rewards to optimize chemical validity and incorporate a lightweight protein embedding projector for end-to-end training. Experimental results on structure-based drug design demonstrate state-of-the-art performance with a Vina score of -7.21, validating our unified multimodal approach for practical drug discovery applications.

==> tables/B-2-qm9.tex <==
\begin{table*}[h!]
\centering


\begin{tabular}{lccccc}
\toprule
\textbf{Method} & \textbf{Atom Sta (\%)} & \textbf{Mol Sta (\%)} & \textbf{Valid (\%)} & \textbf{Unique (\%)} & \textbf{RMSD (↓)} \\
\midrule
Ground Truth & 99.52 &97.06 &100.00 &100.00 & - \\
RDKit & 98.25 & 86.87 & 100.00 & 100.00 & 3.07 \\
\textbf{Chem3DLLM\_smiles} & \textbf{99.45} & \textbf{95.00} & \textbf{100.00} & \textbf{100.00} & \textbf{0.71} \\



\bottomrule
\end{tabular}
\caption{Performance comparison on SMILES-to-3D molecule generation (QM9 dataset)}
\label{tab:smiles_3d_generation}
\end{table*}
